Waveform and Spectrum Management for Unmanned Aerial Systems Beyond 2025

The application domains of civilian unmanned aerial systems (UASs) include agriculture, exploration, transportation, and entertainment. The expected growth of the UAS industry brings along new challenges: Unmanned aerial vehicle (UAV) flight control signaling requires low throughput, but extremely high reliability, whereas the data rate for payload data can be significant. This paper develops UAV number projections and concludes that small and micro UAVs will dominate the US airspace with accelerated growth between 2028 and 2032. We analyze the orthogonal frequency division multiplexing (OFDM) waveform because it can provide the much needed flexibility, spectral efficiency, and, potentially, reliability and derive suitable OFDM waveform parameters as a function of UAV flight characteristics. OFDM also lends itself to agile spectrum access. Based on our UAV growth predictions, we conclude that dynamic spectrum access is needed and discuss the applicability of spectrum sharing techniques for future UAS communications.

==> content/a2g__Jaber_Kakar_s_conflicted_copy_2017-06-02_.tex <==
\section{UAV-to-Ground Communication Channel} 

The simplest imaginable system for UAVs in the segregated airspace
consists of the UAV and the Ground Control Station (GCS) with
exclusive frequency assignment for the UAV-GCS link (downlink) as well as the GCS-UAV (uplink). Based on the actual flight range, we need to differentiate between line-of-sight (LoS)
and beyond-LoS (BLoS) communications. In this paper, we focus on LoS links as a result of SUAVs and MAVs soon dominating the airspace and having limited range.

The most throughput-intensive link is the ATG payload link (for example
video). In addition to throughput, latency is critical for S\& A video links
which need to be relayed to either GCS or ATC for decision support. The most crucial data links in terms of UAV airworthiness are C2 links, which require high reliability and low latency, but lower throughput. Combining these requirements, a flexible wideband communications system seems reasonable. OFDM, in particular, can provide high spectral efficiency, flexible data rates and use more or less spectrum as needed and available.

In this paper, we are thus interested in wideband channel models for ATG links to derive suitable OFDM waveform parameters. SUAVs and MAVs typically operate at altitudes of less than 3,000 m. Commercial applications will predominantly take place in built-up areas. As part of our prior work \cite{Jaber}, we have conducted an exhaustive literature survey on ATG channels (see \cite[Chapter 4]{Jaber} for detail). Out of those conducted wideband measurement campaigns and the availability of information, we believe that measurement results available in \cite{Newhall} best describe fading characteristics of SUAV and MAV channels during the en-route phase. Issues in using the results from \cite{Newhall} are, on the one hand, that no information about the Doppler spread is available. On the other hand, the frequency of 2.05 GHz and the position of the ground station at ground level (GL) are not typical configurations under which future SUAVs and MAVs will operate. %Nevertheless, in this part this model is used due to lack of other feasible alternatives. 
We retrieve a power-delay-profile (PDP) prototype defined by the delay vector $\tau=[0\; 33\; 70\; 115\; 175\; 262\; 405\; 682]$ ns and the normalized power vector $P_{dB}=[0\; -8.7\; -9.6\; -11.3\; -13.4\; -15.2\; -17.0\; -20.2]$. The resulting RMS delay spread for then equals $\sigma_{t}=87.5$ ns. Our PDP prototype is similar to 3GPP's rural area channel model (for default velocities of $v=\{120,180\}$ km/h and classical Jakes Doppler Spectrum) \cite{3GPP}, which suggests a RMS delay spread of $\sigma_{t}=100$ ns.% (as opposed to $\sigma_{t}=87.5$ ns for the specified ATG PDP). %The ATG performance is expected to be similar to that of the Rural Area model. 
 In \cite{Newhall}, a maximum excess delay spread of $\tau_{\max}\approx 1.5$ $\mu$s has been observed.


